Fast Tree-Field Integrators: From Low Displacement Rank to Topological Transformers

We present a new class of fast polylog-linear algorithms based on the theory of structured matrices (in particular low displacement rank) for integrating tensor fields defined on weighted trees. Several applications of the resulting fast tree-field integrators (FTFIs) are presented, including (a) approximation of graph metrics with tree metrics, (b) graph classification, (c) modeling on meshes, and finally (d) Topological Transformers (TTs) (Choromanski et al., 2022) for images. For Topological Transformers, we propose new relative position encoding (RPE) masking mechanisms with as few as three extra learnable parameters per Transformer layer, leading to 1.0-1.5%+ accuracy gains. Importantly, most of FTFIs are exact methods, thus numerically equivalent to their brute-force counterparts. When applied to graphs with thousands of nodes, those exact algorithms provide 5.7-13x speedups. We also provide an extensive theoretical analysis of our methods.

==> algorithm.tex <==
% \vspace{-7mm}
\section{Fast Tree-Field Integrators (FTFI)}
\label{sec:ftfi}

\subsection{IntegratorTrees (ITs) - preliminaries}
\label{sec:it}
In order to support fast integration for various tensor fields $\mathbf{X} 
\in \mathbb{R}^{N \times d_{1} \times ... \times d_{s}}$ defined on a given input tree $\mathcal{T}$, we first design a special data structure, that we refer to as an \textrm{IntegratorTree} (IT). An object of this type is constructed only once per $\mathcal{T}$, regardless of the number of tensor fields used.
An IT is a binary tree. To avoid the confusion, we will refer to its vertices as \textit{nodes}, reserving term $\textit{vertices}$ for those of $\mathcal{T}$. Each node of IT corresponds to the induced sub-tree $\mathcal{S}\mathcal{T}$ of $\mathcal{T}$. For every non-leaf node corresponding to some $\mathcal{S}\mathcal{T}$, a \textit{pivot} point $p$ and two sub-trees: $\mathcal{S}\mathcal{T}_{\mathrm{left}}$ and $\mathcal{S}\mathcal{T}_{\mathrm{right}}$  are constructed. The following needs to be satisfied: 
\vspace{-3mm}
\begin{itemize}
\item $|\mathcal{ST}_{x}| \geq \frac{|\mathcal{S}\mathcal{T}|}{4}$    
for $x \in \{\mathrm{left}, \mathrm{right}\}$,
\item $\mathcal{ST}_{x} \cap \mathcal{ST}_{y} = \{p\}$ ($||$ returns the number of vertices).
\end{itemize}
\vspace{-2mm}
Next lemma shows that every tree $\mathcal{K}$ with $|\mathrm{\mathcal{K}}| \geq 6$ has the above decomposition and it can be efficiently found.
\begin{lemma}[\textbf{pivoting}]
\label{thm:pivot_lemma}
If $\mathcal{K}$ is a tree with $|\mathcal{K}| \geq 6$, then $\mathcal{K}$ admits a decomposition
($\mathcal{K}_{\mathrm{left}}, \mathcal{K}_{\mathrm{right}}, \{p\})$ given above and it can be constructed in \textbf{linear} time. 
\end{lemma}
The algorithmic proof is given in the Appendix (\textcolor{red}{Sec. \ref{sec:pivoting_lemma}}) and uses standard tools from the theory of balanced separators.
The \textit{left child} of the non-leaf node for $\mathcal{ST}$ corresponds to $\mathcal{ST}_{\mathrm{left}}$ and the \textit{right child} to $\mathcal{ST}_{\mathrm{right}}$. In addition to these two pointers, the non-leaf node consists also of six extra fields, partitioned into two groups, one corresponding to its left child and one to its right childs.
The fields corresponding to the left child are as follows:
\vspace{-3mm}
\begin{itemize}
\item \textbf{Left-ids:} an array of the ids (in $\mathcal{ST}$) of those vertices that are in $\mathcal{ST}_{\mathrm{left}}$, mapping the ids of vertices in $\mathcal{ST}_{\mathrm{left}}$ to the original ids in $\mathcal{ST}$ (each sub-tree is locally using as ids consecutive numbers from $0$).
\vspace{-2mm}
\item \textbf{Left-d:} an array of different shortest-path \textbf{d}istances from the pivot point to the vertices in $\mathcal{ST}_{\mathrm{left}}$.
\vspace{-2mm}
\item \textbf{Left-id-d:} an array mapping the ids of vertices (in $\mathcal{ST}_{\mathrm{left}}$) to the indices in \textrm{left-d} of their corresponding distances from the pivot point.
\vspace{-2mm}
\item \textbf{Left-s:} a corresponding array of the ordered sub-\textbf{s}ets of ids (in $\mathcal{ST}_{\mathrm{left}}$) of vertices within a particular distance from the pivot point.
\end{itemize}
\vspace{-2mm}
Fields corresponding to the right child are defined similarly.
The leaf-nodes of the IT consist only of the f-transformed (element-wise) distance matrices $\mathbf{D}$ for their corresponding sub-trees. In principle, the leaf-nodes of IT correspond to sub-trees with less than $t=6$ vertices each. In practice, we can set up any higher $t$, which plays important role in practically-efficient integration (see: \textcolor{red}{Sec. \ref{...}}).
\vspace{-2.5mm}
\paragraph{Time \& space complexity of constructing ITs:} From what we have said so far, it is clear that IT can be constructed by applying \textit{breadth first search} (BFS) and the linear algorithmic procedure for constructing the decomposition from Lemma \ref{thm:pivot_lemma}. Note that every vertex of the input tree appears in the logarithmic number of nodes in the IT, since the size of the sub-tree as we go from the node to its child in IT is reduced by at least the $\frac{1}{4}$ multiplicative factor. We conclude that IT for the given input tree $\mathcal{T}$ can be computed in $O(N\log(N))$ time, where $N$ stands for the number of vertices $|\mathcal{T}|$ of $\mathcal{T}$.
\subsection{Integrating with IntegrationTrees}
\label{sec:int-it}
We are ready to explain how ITs can be applied to conduct efficient integration of the given tensor field $\mathbf{X} \in \mathbb{R}^{N \times d_{1} \times ... \times d_{s}}$ defined on $\mathcal{T}$ for a wide class of function $f:\mathbb{R} \rightarrow \mathbb{R}$. We will apply \textit{divide-and-conquer} strategy. 

We start in the root-node of IT. If that node is a leaf then the $f$-transformed distance matrix is stored and can be directly used for matrix-tensor multiplication. Thus let us assume that this node is not a leaf. But then it encodes the decomposition $(\mathcal{T}_{\mathrm{left}}, \mathcal{T}_{\mathrm{right}},p)$. Note that the value $\mathbf{M}^{\mathrm{G}}_{f}\mathbf{X}[v]$ of the field in $v$ after $f$-integration is given as follows for $\mathcal{W} = \mathrm{V}(\mathcal{T}_{\mathrm{right}}) \backslash \{p\}$:
\begin{equation}
\underbrace{\sum_{j \in \mathrm{V}(\mathcal{T}_{\mathrm{left}})}f(\mathrm{dist}(i,j))\mathbf{X}[j]}_{\mathrm{F}_{\textrm{inner}}(v)} + \underbrace{\sum_{j \in \mathcal{W}}f(\mathrm{dist}(i,j))\mathbf{X}[j]}_{\mathrm{F}_{\textrm{cross}}(v)}
\end{equation}




In order to compute the new values of the field for nodes $v \in \mathcal{T}_{\mathrm{left}}$, one needs to:
\vspace{-2mm}
\begin{enumerate}
\item Compute the contribution to it from $\mathcal{T}_{\mathrm{left}}$ ($\mathrm{F}_{\textrm{inner}}(v)$-terms). This can be done simply by applying recursively the procedure for $\mathcal{T}_{\mathrm{left}}$, which (in the language of IT) means traversing to the left child of the root.
\item Add the so-called \textit{cross-terms} contributions coming from the vertices of $\mathcal{W}$ ($\mathrm{F}_{\textrm{cross}}(v)$-terms).
\vspace{-2mm}
\end{enumerate}

The key observation is that the latter (cross-term) contributions can be retrieved simply by computing $\mathbf{C} \mathbf{X}^{\prime}$, where $\mathbf{C} \in \mathbb{R}^{k \times l}$ with $k$ and $l$ standing for the size of the left-d and right-d array in the node respectively, $\mathbf{C}(i,j)=f(\textrm{left-d}[i]+\textrm{right-d}[j])$, and furthermore $\mathbf{X}^{\prime} \in \mathbb{R}^{l \times d_{1} \times ... \times d_{s}}$ is defined as follows for $b \overset{\mathrm{def}}{=} |\textrm{right-s}[j]|$: 
\vspace{-1mm}
\begin{equation}
\mathbf{X}^{\prime}[j] \overset{\mathrm{def}}{=} \sum_{z=0}^{b-1} \mathbf{X}[\textrm{right-ids}[\textrm{right-s}[j][z]]]
\end{equation}
In the definition of $b$, $||$ refers to the size of the subset. 
We conclude that, given the structure of IT, tensor $\mathbf{X}^{\prime}$ can be computed in linear time. Note that the following holds:
\begin{equation}
\mathrm{F}_{\mathrm{cross}}(v) = \mathbf{C}\mathbf{X}^{\prime}[\tau(v)] - f(\textrm{left-d}[\tau(u)])\mathbf{X}^{\prime}[0],
\end{equation}
where $\tau(v)=\textrm{left-id-d}[v]$.
Analogous analysis can be derived for $v \in \mathcal{T}_{\mathrm{right}}$, with matrix $\mathbf{C}^{\top}$ replacing $\mathbf{C}$.
Thus the overall time complexity of the cross-terms computations is determined by the algorithm for matrix-tensor multiplications with matrices $\mathbf{C}$ and $\mathbf{C}^{\top}$.

\subsubsection{The case for structured matrices: multiplications with $\mathbf{C},\mathbf{C}^{\top}$ and cordiality}
\label{sec:ldr}
Matrices $\mathbf{C},\mathbf{C}^{\top}$ are of the form: $[f(x_{i}+y_{j})]_{i=1,...,a}^{j=1,...,b}$ for some sequences $X=(x_{i})_{i=1}^{a}$, $Y=(y_{j})_{j=1}^{b}$ and $a,b \in \mathbb{N}_{+}$.
\begin{definition}[cordial functions]
\label{def:cordial}
We say that a function $f:\mathbb{R} \rightarrow \mathbb{R}$ is $d$-cordial with respect to $(\mathcal{X},\mathcal{Y})$, where $\mathcal{X}=(X_{1},X_{2},...)$, $\mathcal{Y}=(Y_{1},Y_{2},...)$ are two infinite sequences of non-empty finite sequences, if there exists $d \in \mathbb{N}$ such that matrix-vector multiplication with a matrix $\mathbf{M}=[f(x+y)]_{x \in X_{i}}^{y \in Y_{j}}$ can be conducted in time $O((|X_{i}|+|Y_{i}|)\log^{d}(|X_{i}|+|Y_{i}|))$ for every $i=1,2,...$and where $||$ denotes sequence's length. If this holds for arbitrary: $\mathcal{X}$ and $\mathcal{Y}$, we say that $f$ is $d$-hypercordial (or simply: hypercordial if we do not want to specify $d$).
\end{definition}

Why are cordial functions important for us ? 
\begin{lemma}[$f$-integration with cordial functions]
\label{lemma:cordial}
Assume that $T=(\mathrm{T}_{1},\mathrm{T}_{2},...)$ is a sequence of weighted trees closed under induced connected sub-graph operation. If $f$ is $d$-cordial with respect to $(\mathcal{X},\mathcal{Y})$
where: (1) $\mathcal{X}=(X_{1},X_{2},...)$, $\mathcal{Y}=(Y_{1},Y_{2},...)$, (2) $X_{i}$ and $Y_{i}$ are some sequences containing all distances between vertices in $\mathrm{T}_{i}$ then $f$-integration on $T_{i}$ for $i=1,2,...$ can be conducted in time $C |T_{i}| \log^{d+1}(|T_{i}|)$ for some universal $C>0$.
\end{lemma}
\begin{proof}
...    
\end{proof}

Next we show several practical implications of Lemma \ref{lemma:cordial}.
\paragraph{Function: arbitrary, unweighted tree:}
Define $T$ as a set of all unweighted trees (i.e. with all weights equal to one) and let $X_{i}=Y_{i}=(0,...,|V(T_{i})|-1)$. Note that $f$ is $1$-cordial with respect to $(\mathcal{X},\mathcal{Y})$ since matrix $\mathbf{M} \in \mathbb{R}^{a \times b}$ from Def. \ref{def:cordial} is \textit{Hankel} \citep{hankel} and, as an LDR matrix, supports $O((a+b)\log(a+b))$ matrix-vector multiplication via Fast Fourier Transform (FFT). We conclude that $f$-integration can be conducted in $O(N\log^{2}(N))$ time for $N$-vertex unweighted trees and any $f:\mathbb{R} \rightarrow \mathbb{R}$. This was already proven in \citep{topvit}.
\paragraph{Function: rational, weighted tree:} We claim that every rational $f$ is $(2+\epsilon)$-hypercordial for any $\epsilon>0$. We will use Lemma 1 from \citep{inverse-geo} stating that: given any set of $b$ rational functions $R_{i}(x)=\frac{P_{i}(x)}{Q_{i}(x)}$ of constant degree each, in coefficient representation, and a set of $a$ values $x_{j}$, one can compute the $a$ values $\sum_{i} R_{i}(x_{j})$ in time $O(a+b)\log^{2}(b)\log(\log(b))$ (also by applying FFT). For a given vector $\mathbf{v} \in \mathbb{R}^{b}$, it thus suffices to define: $R_{i}(x)=\sum_{j=1}^{b}v_{b}f(x_{j}+y_{i})$ and that lemma can be applied to efficiently compute $\mathbf{Mv}$. We conclude that $f$-integration can be conducted in $O(N\log^{3+\epsilon}(N))$ time for $N$-vertex weighted trees and any rational $f:\mathbb{R} \rightarrow \mathbb{R}$ and $\epsilon>0$.
 \paragraph{Function: polynomial, weighted tree:} The above result clearly applies also to polynomial $f$, but here we can do better. We show that $f$ is $0$-hypercordial. Assume that $f(x)=\sum_{t=0}^{B} a_{t}x^{t}$. We have: $\mathbf{M}=\sum_{t=0}^{B}\sum_{l=0}^{t} a_{t}{t \choose l} \mathbf{M}_{l,t-l}$, where matrix $\mathbf{M}_{u,v} \in \mathbb{R}^{a \times b}$ is defined as an outer-product of two vectors: $(x_{1}^{u},...,x_{a}^{u}) \in \mathbb{R}^{a}$ and $(y_{1}^{v},...,y_{b}^{v}) \in \mathbb{R}^{b}$. Thus each $\mathbf{M}_{u,v}$ supports linear matrix-vector multiplication (via matrix associativity property). The proof is completed, since $B$ is a constant. We conclude that $f$-integration can be conducted in $O(N\log(N))$ time for $N$-vertex weighted trees and any polynomial $f:\mathbb{R} \rightarrow \mathbb{R}$.
\paragraph{Function: exponential, weighted tree:} Let us assume now that $f(x)=\exp(\lambda x)$. Then $\mathbf{M}$ is an outer-product of two vectors: $(\exp(\lambda x_{1}),...,\exp(\lambda x_{a})) \in \mathbb{R}^{a}$ and $(\exp(\lambda y_{1}),...,\exp(\lambda y_{b})) \in \mathbb{R}^{b}$. The remaining analysis and conclusion is thus the same as for the polynomial case.
\paragraph{Function: exponential $\times$ polynomial, weighted tree:}
Note that a Hadamard (element-wise) product of two outer-product matrices is itself an outer-product matrix. Thus, using the analysis for the two above results (for the exponential and polynomial functions), we conclude that $\mathbf{M}$ is a sum of a constant number of terms, where each is an outer-product matrix, and the same conclusion follows.
\paragraph{Function: $f(x) = \frac{\exp(\lambda x)}{x+c}$, weighted tree:} We claim that $f$ is $1$-hypercordial. In that setting, matrix $\mathbf{M}$ satisfies: $\mathbf{M}(i,j)=\frac{\exp(\lambda x_{i})\exp(\lambda y_{j})}{(x_{i}+\frac{c}{2})+(y_{j}+\frac{c}{2})}$ and thus is a \textit{Cauchy-like} LDR, supporting fast $O(N\log^{2}(N))$ matrix-vector multiplication \citep{cauchy}. We conclude that $f$-integration can be conducted in $O(N\log^{3}(N))$ time for $N$-vertex weighted trees and $f(x)=\frac{\exp(\lambda x)}{x+c}$.
\paragraph{The case of the trigonometric $f$:} If $f(x)=\cos(x)$ then it can be re-written as: $f(x) = \frac{\exp(\mathbf{i}x)+\exp(-\mathbf{i}x)}{2}$. Observe that the cordiality property is preserved under linear combination of the finite number of cordial functions. We can thus conclude that analogous results as the above for $f(x)=\exp(\lambda x)$ can be derived for $f(x)=\cos(x)$. That is also the case for $f(x)=\sin(x)$ that can be re-written as: $f(x) = \frac{\exp(\mathbf{i}x)-\exp(-\mathbf{i}x)}{2\mathbf{i}}$. In both cases, we extend the domain from $\mathbb{R}$ to $\mathbb{C}$, but this does not affect the analysis.

\paragraph{Trees with positive rational weights:} The analysis for the case of arbitrary functions and unweighted trees can be extended to trees with weights taking values in $\{\frac{e}{q}: e \in \{1,...,p\}\}$ for some $p,q \in \mathbb{N}_{{+}}$. This can be done simply by defining: $X_{i}=Y_{i}=\{\frac{l}{q}:l=0,1,...,p(|V(T_{i})|-1)\}$. This does not change asymptotic time complexity, but introduces potentially large multiplicative constant since it increases the number of rows and columns of a matrix $\mathbf{M}$ by a multiplicative constant $p$. 


==> places365_table.tex <==
\begin{table}[t]
    \caption{{Performance of different Topological Vision Transformers with tree-based masking on Places365 dataset. We put in \textbf{bold} the best variant and in \textcolor{blue}{blue} the Performer baselines.}}
    \begin{center}
    \scalebox{0.9}{
     \begin{tabular}[H]{ c c c c c c } 
    \toprule
     $\textbf{\textrm{Dataset}}$
     & $\textbf{\textrm{$\phi$}}$ & $\textbf{\textrm{synced}}$ & $\textbf{\textrm{g}}$ & 
     $\textbf{\textrm{t}}$  & $\textbf{\textrm{Accuracy}}$ (\%)\\ [0.5ex] 
    \midrule
     \multirow{7}{*}{Places365} & 
     \multirow{7}{*}{$\mathrm{ReLU}(x)$}  & 
     $\textrm{NA}$ 
     & $\mathrm{NA}$ & 
     $\mathrm{NA}$ & 
     $\textrm{\textcolor{blue}{54.80}}$ \\
      &   & \xmark & $\exp$ & 
     ~~$\textrm{1}$ & 
     $\textrm{\textbf{56.69}}$ \\
     &   & 
     \xmark 
     & $z \rightarrow z^{-1}$ & 
     ~~$\textrm{1}$ & 
     $\textrm{56.44}$ \\
     & & 
     \xmark 
     & $z \rightarrow z^{-1}$ & 
     ~~$\textrm{3}$ & 
     $\textrm{56.22}$ \\
     &  & 
     \xmark 
     & $z \rightarrow z^{-1}$ & 
     ~~$\textrm{5}$ & 
     $\textrm{56.32}$ \\
     &  & 
     \xmark 
     & $z \rightarrow z^{-1}$ & 
     ~$\textrm{10}$ & 
     $\textrm{56.51}$ \\
     &  & \xmark & $z \rightarrow z^{-1}$ & 
     ~$\textrm{15}$ & 
     $\textrm{56.14}$ \\
    \bottomrule     
    \end{tabular}}
     \label{table:tts-places}
    \end{center}
\end{table}
